Entropy-Enhanced Multimodal Attention Model for Scene-Aware Dialogue Generation

With increasing information from social media, there are more and more videos available. Therefore, the ability to reason on a video is important and deserves to be discussed. TheDialog System Technology Challenge (DSTC7) (Yoshino et al. 2018) proposed an Audio Visual Scene-aware Dialog (AVSD) task, which contains five modalities including video, dialogue history, summary, and caption, as a scene-aware environment. In this paper, we propose the entropy-enhanced dynamic memory network (DMN) to effectively model video modality. The attention-based GRU in the proposed model can improve the model's ability to comprehend and memorize sequential information. The entropy mechanism can control the attention distribution higher, so each to-be-answered question can focus more specifically on a small set of video segments. After the entropy-enhanced DMN secures the video context, we apply an attention model that in-corporates summary and caption to generate an accurate answer given the question about the video. In the official evaluation, our system can achieve improved performance against the released baseline model for both subjective and objective evaluation metrics.

==> attention.tex <==
\subsection{Summary and Caption Attention}
After we reviewed the whole dataset, we found that lots of questions are mostly details in video. Hence, caption and summary were unable to provide applicable information. Nonetheless, after visualizing the model's attention, the attention still are able to extract suitable keyword while both modalities are related to the question. As in Fig.1, question [0] ask "what is the person doing?", which summary and caption basically sums up what it is doing. As a result, the attention attend on "hugging", "pillow", and "laughing". However, other questions are too details that caption and summary do not cover.
\input{attention_figure.tex}



==> attention_figure.tex <==
\begin{figure*}[t!]
  \vspace{-1.5em}
  \centering
  \subfloat[Summary]{\raisebox{-0ex}{ \includegraphics[height=0.25\textheight,width=0.49\textwidth]{figure/summary-attention.png}}\label{fig:f1}}
  \hfill
  \subfloat[Caption]{\includegraphics[height=0.25\textheight,width=0.49\textwidth]{figure/caption-attention.png}\label{fig:f2}}
  \caption{question [0]: what is the person doing? Summary attention focuses on  "hugging" and "pillow". Caption attention focused on "laughing". Caption and Summary aren't able to supply useful information to [1] to [9] Questions. }
  \label{attention_visualization}
  \vspace{-1.6em}
\end{figure*}

